Information Value: Measuring Utterance Predictability as Distance from Plausible Alternatives

We present information value, a measure which quantifies the predictability of an utterance relative to a set of plausible alternatives. We introduce a method to obtain interpretable estimates of information value using neural text generators, and exploit their psychometric predictive power to investigate the dimensions of predictability that drive human comprehension behaviour. Information value is a stronger predictor of utterance acceptability in written and spoken dialogue than aggregates of token-level surprisal and it is complementary to surprisal for predicting eye-tracked reading times.

==> tables/comparison-wallbridge.tex <==
\begin{table*}
\centering
\begin{tabular}{lcc}
\toprule
\textbf{Surprisal estimator}                & \textbf{DailyDialog} & \textbf{Switchboard} \\ \midrule
\textbf{Probabilistic (TurnGPT Small)}      & $\rho$                     &     $\rho$                 \\ 
\textit{Sum}                                & -0.341               & -0.273               \\
\textit{Mean}                               & -0.350               & -0.299               \\
\textit{Relative}                           & -0.360               & -0.262               \\
\textit{Max}                                & -0.407               & -0.400               \\
\textit{Variance}                           & -0.295               & -0.217               \\ \midrule
\textbf{Alternative-based (DialoGPT Small)} &                      &                      \\ 
\textit{Mean Lexical Distance}              & 0.103*               & -0.074*              \\
\textit{Min Lexical Distance}               & -0.331                & -0.265                   \\
\textit{Mean Syntactic Distance}            & 0.172*                & -0.070                  \\
\textit{Min Syntactic Distance}             & -0.304                & -0.408                  \\
\textit{Mean Semantic Distance}             & -0.430               & -0.587               \\
\textit{Min Semantic Distance}              & -0.463               & -0.623               \\ \bottomrule
\end{tabular}
\caption{Spearman correlation with median acceptability judgements. Asterisk indicates $p$-value higher than 0.05.}
\label{tab:comparison-wallbridge}
\end{table*}

==> tables/surprisal-joint-lme.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
                  & \swb & \dd & \provo \\ \midrule
\textbf{Surprisal}         & 6.63               & 5.08               & 59.04                 \\
\textbf{Information value} & 43.11               & 35.42              & 45.19                 \\
\textbf{Joint}             & 44.11               & 30.55              & 93.08                \\ \bottomrule
\end{tabular}%
}
\caption{\deltall\ for surprisal, information-value (lexical, syntactic, and semantic), and joint models.}
\label{tab:surprisal-comparison-joint}
\vspace{-12pt}
\end{table}

==> tables/surprisal_iv_joint_lme.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
                            & \swb   & \dd      & \provo \\ \midrule
\textbf{Information value}  & 43.11  & 35.42    & 45.19                \\
\textbf{Surprisal}          & 6.63   & 5.08     & 59.04                \\
\midrule
\textbf{   $+$ lexical}     & x.xx   & x.xx     & x.xx                 \\
\textbf{   $+$ syntactic}   & x.xx   & x.xx     & x.xx                 \\
\textbf{   $+$ semantic}    & x.xx   & x.xx     & x.xx                 \\
\textbf{   $+$ all (Joint)} & 44.11  & 30.55    & 93.08                \\ 
\bottomrule
\end{tabular}%
}
\caption{\deltall\ for surprisal, information-value, and joint models including ablations of the lexical levels of information value.}
\label{tab:surprisal-comparison-joint}
\vspace{-12pt}
\end{table}
